Integrating Learning and Reasoning with Deep Logic Models

Deep learning is very effective at jointly learning feature representations and classification models, especially when dealing with high dimensional input patterns. Probabilistic logic reasoning, on the other hand, is capable to take consistent and robust decisions in complex environments. The integration of deep learning and logic reasoning is still an open-research problem and it is considered to be the key for the development of real intelligent agents. This paper presents Deep Logic Models, which are deep graphical models integrating deep learning and logic reasoning both for learning and inference. Deep Logic Models create an end-to-end differentiable architecture, where deep learners are embedded into a network implementing a continuous relaxation of the logic knowledge. The learning process allows to jointly learn the weights of the deep learners and the meta-parameters controlling the high-level reasoning. The experimental results show that the proposed methodology overtakes the limitations of the other approaches that have been proposed to bridge deep learning and reasoning.

==> impl.tex <==
%root=weight_learning.tex

\subsection{Mini-batch Learning}
It is fundamental to think of a way of allowing the model to work in a mini-batch learning fashion. This would allow the framework to be extended to:
\begin{enumerate}
 \item larger datasets, both in terms of number of individuals and number of relations;
  \item more complex logic programs, where the complexity of a logic program, in our fuzzy setting, is exponential in the maximum number of variables contained in the formulas (since it has to evaluate formulas on the Cartesian product of their domains)
\end{enumerate}

For the sake of simplicity, let us hypothesize that the environmental constraints are \textit{local} constraints, i.e. they do not depend on the general structure of the data. For example, if the environmental constraint is mapping the value of a binary relation on two specific constants to the output of a neural network, then it will depend only on the two constants.

On the contrary, the logical constraints are intrinsically global, since, in most of the cases, they are universally or existentially quantified formulas. However, there is a nice feature of DLM when compared to other systems (e.g. SBR), that is: logical constraints weights are learned in a local constrastive fashion. In particular, focusing on Equation~\ref{eq:lambda_gradient}, we see that the lambdas are updated only of a quantity proportional to the difference between the rules satisfaction on the training data and the rule satisfaction on the MAP solution. 

But following arguments similar to the ones inspiring Stochastic Gradient methods, we can say that if the rules satisfaction on the MAP state is related \textit{only} to a portion of the data, we can still stochastic-ally learn meaningful weights, since only the difference with the rules satisfaction on the same portion of training data is important.
   

==> map.tex <==
MAP inference assumes that the logic and environmental constraint weights are fixed and it aims at finding the assignment maximizing $p(\B y |  X; \B \lambda, \B w)$. MAP inference does not require to compute the partition function $Z$ which acts as a constant when the weights are fixed. Therefore:
\begin{align*}
{\bf y}_M & = \text{arg}\!\max_{\bf y} \log p({\bf y} | X; \B w, \B \lambda) \\
& = 
\text{arg}\!\max_{\bf y}\bigg [ \sum_\ell \phi_\ell(\B y,\lambda_\ell) + \sum_e \phi_e(\B y,\B X,\B w_e)\bigg ].
\end{align*}

The above maximization problem can be optimized by gradient descent by computing the gradient:
$$
\nabla_{\bf y}\log p = \sum_\ell \lambda_\ell \nabla_{\bf y} \psi_c(\B y) + \nabla_{\bf y} \phi_{e}(\B y, \B X; \B w)
$$




==> train.tex <==
Weight learning can be formulated as a maximum log-likelihood problem on the train data ${\bf y}_t$, where we can alternate optimization with respect to the logical constraint weights $\B \lambda$ and the environmental constraint weights $\B w$. In particular, we want to solve the following optimization problem:

\begin{align*}
\B \lambda^\star, \B w^\star = \text{arg}\max_{\B \lambda, \B w} \log p(\B y_t | \B X;\B \lambda, \B w)
\end{align*}

Now, we calculate the derivatives of $p(\B y_t | \B X;\B \lambda, \B w)$  with respect to $\B \lambda$ and $\B w$, respectively. For what concerns logical constraint weights, we have:
\begin{align*}	
	\frac{\partial \log p}{\partial \lambda_\ell}
	&= \psi_\ell({\bf y}_t) - \frac{\partial \log Z}{\partial \lambda_\ell} 
	\psi_\ell({\bf y}_t) - \frac{1}{Z} \frac{\partial Z}{\partial \lambda_\ell} \\
	&= \psi_\ell({\bf y}_t) - \frac{\partial }{\partial \lambda_\ell} \int \frac{1}{Z} \exp\left(\sum_\ell \lambda_\ell \psi_\ell({\bf y}^\prime))) + \sum_e \phi_e({\bf y}^\prime, \B X; \B w))\right) d{\bf y}^\prime  \\
	&= \psi_\ell({\bf y}_t) - \int \frac{\exp\left(\sum_\ell \lambda_\ell \psi_\ell({\bf y}^\prime))) +  \sum_e \phi_e({\bf y}^\prime, \B X; \B w)))\right)}{Z} \psi_\ell({\bf y}^\prime) d{\bf y}^\prime  \\
	&= \psi_\ell({\bf y}_t) - \int p({\bf y}^\prime | \B w, X) \psi_\ell({\bf y}^\prime) d{\bf y}^\prime  \\
	&= \psi_\ell({\bf y}_t) - E_p[\psi_\ell].
\end{align*}


Unfortunately, the computation of the expected value $E_p[\psi_\ell]$ requires to iterate over all possible assignments and it needs to be approximated.
A common assumption is that the MAP solution dominates the integral of the partition function, namely:
\begin{align}
p({\bf y} | X; \B \lambda, \B w) = \delta({\bf y} - {\bf y}_M)
\label{eq:approx}
\end{align}

As a result, we get:
\begin{align}
\label{eq:lambda_gradient}
	\frac{\partial \log p}{\partial \lambda_\ell} &= \psi_\ell({\bf y}_t) - E_p[\psi_\ell] \approx \psi_\ell({\bf y}_t) - \int \delta({\bf y}^\prime - {\bf y}_M) \psi_\ell({\bf y}^\prime) d{\bf y}^\prime \nonumber \\ 
	&= \psi_\ell({\bf y}_t) - \psi_\ell({\bf y}_M)
\end{align}

%\begin{equation}
%Z \approx \exp\left(
%\sum_c \lambda_c \phi_c({\bf y}_M) +
%\phi_e({\bf y}_M, f_{\B w}(X))
%\right)
%\end{equation}

While this approximation is often considered too weak in the context of working with exponential models, we will justify it in the following of the paper. DA FAREEEEEEEEEE. PROBABILMENTE LA PARTE DI MAP AS APPROXIMATED INFERENCE DEL DOC  OVERLEAF PUO' ESSERE UTILE

We can use similar arguments for the computation of derivatives w.r.t. environmental constraint weights. In particular, we have:
\begin{align*}
	\frac{\partial \log p}{\partial w_{i}} =& \frac{\partial}{\partial w_{i}} \sum_e \phi_e({\bf y}^\prime, \B X; \B w) - E_p\left [\frac{\partial}{\partial w_{i}}\sum_e \phi_e({\bf y}^\prime, \B X; \B w)\right ]
\end{align*}
	
	

Using the same approximation for the expected value used before, yields: 
\begin{align*}
	\frac{\partial \log p}{\partial w_{i}} & \approx\frac{\partial}{\partial w_{i}} \sum_e \phi_e({\bf y}^\prime, \B X; \B w) - \frac{\partial}{\partial w_{i}}\sum_e \phi_e({\bf y}_M, \B X; \B w)\\
	& = \frac{\partial}{\partial w_{i}} \sum_e (\phi_e({\bf y}^\prime, \B X; \B w) - \phi_e({\bf y}_M, \B X; \B w))
\end{align*}

When some of the environmental constraints are modelled as deep architectures, a step of backpropagation is triggered. 

 
The weight learning process consists in applying a gradient descent approach exploiting the derivatives previously computed. However, the approximation performed in computing the gradient, while simplifying extremely the computations, still needs a MAP inference task to compute the MAP state $\B y_M$  required to update of the parameters. In these terms, the MAP inference can be devised as a building block of the learning process.  Thus, we are in front of an EM procedure where we alternate \textit{(E)}, where we compute MAP state given the current parameters, and\textit{(M)}, where we maximize the probability of training data by updating the parameters. The process is described in Algorithm \ref{alg:learning}.



\paragraph{Loss Function} Even though the approximation in Eq. \ref{eq:approx} is performed during the computation of the derivatives, we can design a loss function whose minimization leads exactly to the same learning dynamics. This loss function can be interpreted as an approximated negative log-likelihood and it can be defined as follows:

\begin{align*}
\mathcal{L}(\B y_t, \B y_M, \B X, \B \lambda, \B w) = \sum_\ell \lambda_\ell \big (\psi_\ell(\B y_M) - \psi_\ell(\B y_t)\big ) + \sum_e (\phi_e({\bf y}_M, \B X; \B w) - \phi_e({\bf y}_t, \B X; \B w))
\end{align*}


Demonstrating the equality between the derivatives of this function and the approximated ones of the log-likelihood is straightforward. However, this loss function makes it clearer what the learning process is trying to achieve. In particular, it is trying to learn those weights such that the level of satisfaction of the constraints is equal on both the MAP state and the training data, which is absolutely reasonable. The state to which the model assigns the maximum probability should be the one that is mostly coherent with the training data.


\paragraph{Lagrangian Formulation} %vedi se c'è un legame più preciso a livello di teoria..
The joint learning of parameters and MAP inference can also be formulated in a Lagrangian perspective, where Lagrange conditions provide some convergence conditions so that an optimal solution is reached in algorithm \ref{alg:bo}. The optimization problem can be expressed as,
\begin{eqnarray*}
\begin{array}{l}
\displaystyle\min_{{\bf y}, {\bf w}} \Phi_e({\bf y},f(X))-\Phi_e({\bf y}_t,f(X))\\
\\
\texttt{subject to:} \\
\psi_\ell({\bf y}_t) = \psi_\ell({\bf y}) ~~ \forall \ell\in L
\end{array}
\end{eqnarray*}
The distance between ${\bf y}$ and $f(X)$ has to be equal to the distance between ${\bf y}_t$ and $f(X)$, while satisfying the logical constraints. An optimal solution for this problem is given by a saddle point of $\mathscr{L}$, namely solving
\[
\max_{\lambda}\min_{{\bf y},{\bf w}} \mathscr{L}({\bf y},{\bf w},\lambda)
\]
where $\lambda$ denotes the vector of Lagrangian multipliers and
\[
\mathscr{L}({\bf y},{\bf w},\lambda)=\Phi_e({\bf y},f(X))-\Phi_e({\bf y}_t,f(X))+\sum_{\ell\in L}\lambda_\ell\left(\psi_\ell({\bf y}) - \psi_\ell({\bf y}_t)\right) \ .
\]
As in the case of model (\ref{eq:model}), the gradients of  $\mathscr{L}$ are given by
\[
\begin{array}{l}
\frac{\partial \mathscr{L}}{\partial {\bf y}} =
\nabla_{\bf y}\Phi_e({\bf y},f(X)) + \sum_{\ell\in L} \lambda_l \nabla_{\bf y}\psi_\ell({\bf y}) 
\\
\\
\frac{\partial \mathscr{L}}{\partial w_i} =
\big(\nabla_{\bf y}\Phi_e({\bf y},f(X)) - \nabla_{\bf y}\Phi_e({\bf y}_t,f(X))\big)\cdot \frac{\partial f(X)}{w_i}\\
\\
\frac{\partial \mathscr{L}}{\partial \lambda_\ell} = \psi_\ell({\bf y}_t) - \psi_\ell({\bf y})
\end{array}
\]
and optimal solutions are determined by such points annulling the gradient of $\mathscr{L}$ while satisfying the constraints.



\paragraph{Adversarial Learning} There is a nice interpretation of the dynamics of Algorithm \ref{alg:learning} in terms of an adversarial learning procedure. To show this interpretation, let us start to notice the equivalence between these two optimization problems:

\begin{align*}
{\bf y}_M & = \text{arg}\!\max_{\bf y} \log p({\bf y} | X; \B w, \B \lambda)  = \text{arg}\!\max_{{\bf y}_m} \mathcal{L}(\B y_t, \B y_m, \B X, \B \lambda, \B w)
\end{align*}
since all the terms in $\mathcal{L}$  depending on $\B y_t$ are constant w.r.t. $\B y_m$.

Thus, MAP inference and parameter training are respectively trying to maximize and minimize the same loss function in an adversarial fashion. MAP inference is discovering maximum probability masses which are far from the unknown data model while parameter learning is trying to decrease the probability mass in those areas. This process iterates until the model gives the maximum probability to the data. 

It must be clear that the exploration of the $\B y$ space of the proposed approach is still  limited and it can happen that the model assigns high probability to areas far from the data region (i.e. we are decreasing only \textit{maximum} probability masses far from data). However, the presence of the environmental constraints ensures that most of the areas far from the manifold induced by $\B X$ are automatically assigned a low probability, allowing our approach to still reach very good results in discriminative settings, as shown in the following sections.
